kNN-Prompt: Nearest Neighbor Zero-Shot Inference

Retrieval-augmented language models (LMs) use non-parametric memory to substantially outperform their non-retrieval counterparts on perplexity-based evaluations, but it is an open question whether they achieve similar gains in few- and zero-shot end-task accuracy. We extensively study one such model, the k-nearest neighbor LM (kNN-LM), showing that the gains marginally transfer. The main challenge is to achieve coverage of the verbalizer tokens that define the different end-task class labels. To address this challenge, we also introduce kNN-Prompt, a simple and effective kNN-LM with automatically expanded fuzzy verbalizers (e.g. to expand terrible to also include silly and other task-specific synonyms for sentiment classification). Across nine diverse end-tasks, using kNN-Prompt with GPT-2 large yields significant performance boosts over strong zero-shot baselines (13.4% absolute improvement over the base LM on average). We also show that other advantages of non-parametric augmentation hold for end tasks; kNN-Prompt is effective for domain adaptation with no further training, and gains increase with the size of the retrieval model.

==> sections/experiment.tex <==
\input{tables/data_info}

\section{Experimental Setup}

% \subsection{Verbalizer construction} \label{sec:verbalizer-construction}
% \todo{[Julian: I this section should be moved much later into an 'experiments' subsection since in Methods we're just describing the general approach independent of any particular task. We should keep the task-specific details all in one place later in the paper. Maybe even some of the details in the earlier section can go there too, we'll see.}
%Previous studies~\cite{holtzman-etal-2021-surface, zhao2021calibrate} show that verbalizers have a great impact on language models' zero-shot performance. 
%Moreover, as explained in section~\ref{datastore}, our datastore only saves contexts where the next token belongs to the set of label words. Therefore, we need to select a comprehensive and diverse set of label words to fully leverage the power of \ourmodel. 
%Existing works on zero-shot learning~\cite{schick-schutze-2021-exploiting, holtzman-etal-2021-surface} use handcrafted verbalizers, which have limited coverage and require domain expertise. Some other works design automatic verbalizer search~\cite{gao-etal-2021-making, shin-etal-2020-autoprompt, schick-schutze-2021-exploiting} that automatically finds suitable label words, but they require training data for learning the verbalizer.
%As we consider zero-shot scenarios where training data is not available, we leverage different external sources such as WordNet synsets, sentiment dictionary, knowledge bases and word embeddings to expand label word sets in sentiment analysis and topic classification tasks. 
% For topic classification, we rely on GloVe word embeddings~\cite{pennington-etal-2014-glove} and knowledge bases such as ConceptNet~\cite{speer2017conceptnet} to find label words related to a topic.
% Starting from a topic name $v$, we extract top-k similar words $W_g(v)$ using the cosine similarity of GloVe word vectors and collect related terms $W_c(v)$ from ConcepNet~\footnote{https://conceptnet.io/}. 
% Thus, the verbalizer in topic classification maps a set of label words $V_y = y \cup W_g(v) \cup W_c(v)$ to a label $y$. 
% For sentiment analysis, we follow a prior work ~\cite{hu2021knowledgeable} and use sentiment dictionaries as label word sets. ~\footnote{https://enchantedlearning.com/wordlist/positivewords.shtml} ~\footnote{https://enchantedlearning.com/wordlist/negativewords.shtml} 
% We further expand label words set by youextracting synonyms of these words using WordNet synsets. 

\subsection{Datasets and verbalizer construction} \label{sec:verbalizer-construction}
We perform experiments on 11 tasks, including fact retrieval, QA, topic classification, sentiment analysis, entailment and partisanship classification. We briefly describe each dataset and its verbalizer construction process. We collect additional label words for topic classification and sentiment analysis by leveraging external knowledge, while QA, fact retrieval and entailment tasks only use label words defined in the task description.  The prompt for each task is shown in Appendix X, along with an example instance.

\textbf{Topic Classification}
We use AG'S News (AGN)~\cite{zhang2015character} for 4-way news topic classification and Yahoo~\cite{zhang2015character} for 10-way question topic classification. For topic classification, we rely on GloVe word embeddings~\cite{pennington-etal-2014-glove} and knowledge bases such as ConceptNet~\cite{speer2017conceptnet} to find label words related to a topic.
Starting from a topic name, we extract top-k similar words using the cosine similarity of GloVe word vectors and collect related terms from ConcepNet~\footnote{https://conceptnet.io/}. The top-k similar words, related terms along with the original topic name constitute the label word set. 

\textbf{Sentiment and Partisanship}
We study sentiment analysis using Yelp~\cite{zhang2015character}, IMDB, Movie Review (MR)~\cite{pang-lee-2005-seeing} and Customer Review (CR)~\cite{10.1145/1014052.1014073}.IMDB and MR consist of reviews about movies, while CR and Yelp contains a collection of Amazon product reviews and Yelp reviews. Hyperpartisan news detection (HYP)~\cite{kiesel-etal-2019-semeval} focuses on classifying whether a text exhibits prejudiced, or unreasoning allegiance to one party. To collect label words, we follow a prior work ~\cite{hu2021knowledgeable} and use sentiment dictionaries as label word sets.~\footnote{https://enchantedlearning.com/wordlist/positivewords.shtml}~\footnote{https://enchantedlearning.com/wordlist/negativewords.shtml} 
We further expand label words set by extracting synonyms of these words using WordNet synsets. 

\input{tables/main_table.tex}

% SST-2, IMDB and MR consist of reviews about movies, while CR contains a collection of reviews about Amazon product. Hyperpartisan news detection (HYP)~\cite{kiesel-etal-2019-semeval} focuses on classifying whether a text exhibits prejudiced, or unreasoning allegiance to one party. 

\textbf{Entailment}
Entailment dataset focuses on classifying whether the relation between two text segments are entailment or not entailment. We consder Recognizing Textual Entailment (RTE)~\cite{dagan_dolan_magnini_roth_2010} for evaluation. 

\textbf{Fact Retrieval}
We evaluate fact retrieval with LAMA probe~\cite{petroni-etal-2019-language}. The dataset converts subject-relation-object triples into a cloze format which is used to query the language model for a missing token (e.g: Dante was born in [Mask]). Following ~\citeauthor{zhao2021calibrate}, we use test examples where the missing token is at the end of the sentence (suitable for left-to-right LMs). The answer can be any string, which forms an "open set" label space. We report mean accuracy across all triples.

\textbf{Question Answering}
We consider question answering using three datasets, CommonsenseQA (CQA)~\cite{talmor-etal-2019-commonsenseqa}, 
% Open Book Question Answering (OBQA)~\cite{mihaylov-etal-2018-suit}, 
Boolean Question Answering (BoolQ)~\cite{clark-etal-2019-boolq}. CQA consists of multi-choice commonsense questions, which are authored by crowd-workers based on knowledge encoded in ConceptNet~\cite{speer2017conceptnet}. 
% Similar to CQA, OBQA is a multi-choice QA dataset whose answer is based on the knowledge encoded in a set of elementary level science facts. 
% \todo{not sure if we do experiments where }
Because CQA test set is not public, we report accuracy on its development set. BoolQ is a reading comprehension dataset of yes/no questions where each example has a question, an excerpt from a passage and a boolean answer. CQA have open-set labels while BoolQ has only two labels -- yes and no. 

% We consider question answering using three datasets, CommonsenseQA (CQA)~\cite{talmor-etal-2019-commonsenseqa}, 
% % Open Book Question Answering (OBQA)~\cite{mihaylov-etal-2018-suit}, 
% Boolean Question Answering (BoolQ)~\cite{clark-etal-2019-boolq}. CQA consists of multi-choice commonsense questions, which are authored by crowd-workers based on knowledge encoded in ConceptNet~\cite{speer2017conceptnet}. 
% Similar to CQA, OBQA is a multi-choice QA dataset whose answer is based on the knowledge encoded in a set of elementary level science facts. 
% % \todo{not sure if we do experiments where }
% Because CQA test set is not public, we report accuracy on its development set. BoolQ is a reading comprehension dataset of yes/no questions where each example has a question, an excerpt from a passage and a boolean answer. CQA and OBQA have open-set labels while BoolQ has only two labels -- yes and no.



% \subsection{Datastore Corpus}
% We use the following corpus for the datastore.

\subsection{\ourmodel~Model Details}
\noindent \textbf{Inference Model} Since \ourmodel~ makes no change to inference models, we directly use GPT-2 large from Huggingface~\footnote{https://github.com/huggingface/transformers} library as the inference model to conduct zero-shot predictions. 
% We consider 4 different sizes of GPT-2 (small, medium, large and XL) to conduct zero-shot predictions. 

\noindent \textbf{Retriever and Datastore} \ourmodel~is compatible with any language model as a retriever that produces fixed size context representations. Following inference model, we use GPT-2 large for building the datastore. They keys are the 1280-dimensional representation input to the final layer of the model. We run a single forward pass over datastore corpus to save all the keys and values. For efficient similarity search, we create FAISS~\cite{johnson2019billion} index to represent the datastore and search for nearest neighbours.  
% For computational efficiency, we use a small-size model GPT-2 small as the retriever to encode queries and contexts. 
% The with 768 dimensional hidden states  

\subsection{Baselines}
In this subsection, we discuss the baselines we compare with, including continuing pretraining the language model on the corpus cached in the datastore and prepending retrieved contexts in the input. For each baseline, we consider two scoring strategies: a standard method \textit{LM} that simply selects the highest probability option $\hat{y} = argmax \big( \sum_{\mathbf{z} \in \mathbf{Z}_y}{P(\mathbf{z} \mid p(\mathbf{x}) \big)}$, and zero-shot calibration method \textit{PMI} that factors out the probability of surface forms $\hat{y} = argmax\big( \sum_{\mathbf{z} \in \mathbf{Z}_y} \frac{P(\mathbf{z} \mid p(\mathbf{x}))}{P(\mathbf{z} \mid \mathbf{x}_{domain})} \big )$. 

\noindent \textbf{Base} is the original GPT-2 large without the datastore. 

\noindent \textbf{Pretrain}~\cite{gururangan-etal-2020-dont} is a widely-used method to transfer language models to new domains. It continues pretrainining the Base model on the corpus cached in the datastore.

\noindent \textbf{kNN-LM}~\cite{Khandelwal2020Generalization} is the original kNN-LM as shown in ...

\noindent \textbf{Prepend} incorporates examples retrieved by \ourmodel~in a different way by directly prepending them to the input. Each prepended example is formed by concatenating its leftward context and its target token. Because of the context window size limit, we use top 8 retrieved examples in this model.  





\section{Experimental Results}
% \subsection{Domain Adaptation}
We measure the effectiveness of \ourmodel~for domain adaptation, in which we use a domain-specific datastore to adapt the model, without further training. 


We consider three domain-specific corpus: Wikitext-103~\cite{merity2016pointer}, Amazon review corpus~\cite{he2016ups} and a subset of CC-NEWS~\footnote{https://huggingface.co/datasets/cc\_news} and encode each of them in the datastore. Table \ref{data_info} lists the specfics of domain-specific datastores and their target tasks. 

% \todo{change the datastore model: gpt2-s --> gpt2-l}
% \subsection{Results}
Table~\ref{main_table} shows the performance of baselines and \ourmodel. 

\noindent \textbf{\ourmodel~vs. Base}
We observe that \ourmodel~outperform Base consistently for all datasets across both scoring strategies. The average improvements across all datasets are 17.8\% and 12\% for LM and PMI respectively. 
Among all datasets, the largest gains are achieved on CR and LAMA, which can be attributed to the high domain similarity between test set and datastore corpus.

\noindent \textbf{\ourmodel~vs. Prepend} \ourmodel~is always better than Prepend, by xx\% when macro-averaged across all datasets. It suggests that interpolation is a better way to incorporate the retrieved information into language models. We conjecture that the Prepend model may suffer when prepended example have semantically similar leftward context but with target tokens belonging to different label word sets, thus confuse the discriminablity of the model. 

\noindent \textbf{\ourmodel~vs. Pretrain}  
Compared with Pretrain, \ourmodel~achieves much better performance with \textit{LM} and performs comparably with \textif{PMI}. It is interesting to notice that continuing pretraining on in-domain data leads to performance degradation of \textit{LM} on most of the tasks, implying that continuing pretraining exacerbates surface form competition problem. 
% comparable performance than better performance than Pretrain on 9 of 11 tasks and is slightly worse than Pretrain on CR and Yelp in terms of PMI. 
Although PMI is improved by similar amount using Pretrain and \ourmodel, 
% continue pretraining improves Base by similar improvement as 
\ourmodel~
% , different from Pretrain, 
does not require further training, which is more practical and efficient for adapting a very large language model. 
% demonstrating the effectiveness of \ourmodel for easy domain adaptation with no further training. 


% The pattern is consistent across different sized inference models.
%16.2/12.5\% for GPT-2 small, 12.6/6.7\% for medium, 17.8/11\% for large, and 14.7/7.2\% for XL,
 
% the effectiveness of smaller inference model can benefit more from the 

% \noindent \textbf{Impact of inference model size} The average improvements across all datasets using LM are 16.2\% for GPT-2 small, 12.6\% for medium, 17.8\% for large, and 14.7\% for XL. It demonstrates that \ourmodel~consistently improve different sized inference models and GPT-2 Large model benefits most from incorporating kNN distribution. 


% \noindent \textbf{Scoring strategies} PMI is better than LM by a large margin on most datasets. The improvements brought by \ourmodel~ can further improve PMI with 





% \section{Task Adaptation}



% \todo{give explanation on how we choose the datastore?}
% \todo{similar data, less data}knn

==> sections/method.tex <==
\section{Method}

To perform zero-shot predictions on a downstream task using a pretrained language model, we recast the task as language modeling \citep{radford2019language} using prompting together with pre-specified mappings, or \textit{verbalizers}, from the label space into token sequences (\autoref{sec:prompting}).
We then augment the pretrained model with the $k$-nearest-neighbors language modeling technique from \citet{Khandelwal2020Generalization} using a data store that is in-domain for the task (\autoref{sec:knnlm}).
Finally, we decode the output label by applying the \textit{domain-conditional PMI} scoring method of \citet{holtzman-etal-2021-surface} to the resulting language model (\autoref{sec:scoring}). 

\subsection{Prompting and Verbalizers} 
\label{sec:prompting}
Our problem setting is text classification.
Concretely, an instance consists of an input sequence of tokens $\mathbf{x} = (x_0, x_1, ..., x_{|x|})$ from a vocabulary $V$ and an output label $y \in Y$, where $Y$ is a set of possible output labels. 
% For example, as shown in 
Figure~\ref{fig:knn_prompt} shows a sentiment analysis example where the input sequence of tokens is $\mathbf{x}=$"Mr. Tsai is one of world cinema 's most gifted artists." and the set of output labels are $Y$=\{positive, negative\}.
% assuming we need to classify the sentence 
% $\mathbf{x}=$"Mr. Tsai is one of world cinema 's most gifted artists." into one of labels $Y$=\{positive, negative\}.
% \todo{maybe start sentiment example here} 

To cast the task as language modeling, we deterministically transform each input example $\mathbf{x}$ into a \textbf{prompt} $p(\mathbf{x})$. In the above example, $p(\mathbf{x})$ = "Mr. Tsai is one of world cinema 's most gifted artists. It was".
% \todo{elaborate sentiment example}.
This prompt can then be provided to a language model, which assigns a probability $P(\mathbf{z} \mid p(\mathbf{x}))$ to every continuation sequence $\mathbf{z} \in V^*$.
To extract an output label from these continuations, we extend the \textit{verbalizers} of \citet{schick-schutze-2021-exploiting,schick-schutze-2021-just} which map each output label $y \in Y$ to a token in $V$ (e.g., mapping the \textit{positive} sentiment label to the word \textit{good}).
Instead, our verbalizers map each output label $y$ to a set of sequences $\mathbf{Z}_y \subseteq V^*$.
For example, a verbalizer for sentiment analysis might have $\mathbf{Z}_\text{positive} = \{\text{good, excellent, just fantastic }\dots\}$ and $\mathbf{Z}_\text{negative} = \{\text{bad, horrible, no good, }\dots\}$.
Using this, we map the language model's output into a probability distribution over labels as follows:
\begin{equation} \label{eq:prompt-label-prob}
P(y \mid \mathbf{x}) = \frac{\sum_{\mathbf{z} \in \mathbf{Z}_y} P_\text{LM}(\mathbf{z} \mid p(\mathbf{x}))}{\sum_{y \in Y} \sum_{\mathbf{z} \in \mathbf{Z}_y} P_\text{LM}(\mathbf{z} \mid p(\mathbf{x}))}.
\end{equation}
This more general formulation allows us to include words with multiple wordpieces, cover multiple-choice questions (where the label set varies for each input and usually consists of phrases; here we set $\mathbf{Z}_y = \{ y \}$), and improve performance with larger sets of label words.\footnote{Using a larger set of words or phrases for each label will be particularly important for $k$-nearest-neighbor models, since each individual word will be relatively sparse in the data store so it is important to aggregate signal across multiple; see \todo{experiment showing this?}.}
In the zero-shot setting, verbalizers must be determined without reference to training data. For simple verbalizers mapping each output label to a single token, as in past work, it is straightforward enough to specify them manually.
Since we are interested in using multiple words or phrases for each label, we turn to external resources to curate our verbalizers.
More details on how we construct verbalizers for each of our downstream tasks are provided in \autoref{sec:verbalizer-construction}.

%Following previous works on zero-shot classification~\cite{holtzman-etal-2021-surface, zhao2021calibrate}, we converted NLP tasks into human-readable prompted forms.
% ... snip ...
%We wrap the input sequence with a template called prompt $p = (p_0, p_1, ..., p_{|p|})$ to formalize the final input: 
%$$x_{input} = x_0, ..., x_{|x|}, p_0, ..., p_{|p|}$$
%Then a language model $L$ with vocabulary $V$ takes $x_{input}$ as a input to generate a probability distribution of each word $v$ in the vocabulary being the next token. To map the probability of the next token to probability of labels, we define a verbalizer $f$ that learns a mapping from words to labels (i.e: $f: V \rightarrow Y$). For any label $y \in Y$, its probability is computed as:
%\begin{equation*} \label{eq:sum}
%P(y|x_{input}) = \sum_{v \in V_y}{P(v | x_{input})}
%\end{equation*}
% $$P(y|x_{input}) = \sum_{v \in V_y}{P(v | x_{input})}$$ 
%where $V_y$ is the set of tokens corresponding to the label $y$. We use $\cup_{y \in Y} V_y$ to represent subset of tokens in $V$ that can map to a label. In the example in Figure X, previous works may define $V_{positive} = \{good\}$ and $V_{negative} = \{bad\}$. If the probability of "good" larger than "bad", the predicted label will be positive. In our project, we propose to improve the verbalizer by augmenting label word sets using method introduced in section \ref{verbalizer_cons}. Then multiple tokens can be mapped to each class (i.e: $V_{positive} = \{good, great, excellent...\}$). 



%finding similar words of original label words to


% sentiment analysis: sentiment dictionary: \url{https://www.enchantedlearning.com/wordlist/positivewords.shtml}
% \url{https://www.enchantedlearning.com/wordlist/negativewords.shtml}


\subsection{$k$-Nearest Neighbors Language Modeling}
\label{sec:knnlm}

We extend our pretrained language model with the $k$-nearest-neighbors language modeling ($k$NN-LM) approach of \citet{Khandelwal2020Generalization}.
This method augments a language model with a \textit{datastore} from which it can retrieve tokens that inform its predictions, improving performance without further training.

The \textit{datastore} is a key-value store generated by running the language model over a corpus of text.
Each value is a token $w$ from the corpus, and its key is the (vector) hidden representation at the output layer of the language model running forward on $w$'s leftward context $c$ (call this $f(c)$).
At inference time, when predicting the next token for an input sequence $c$, the $k$NN language model retrieves the $k$ nearest neighbors of $c$ from the datastore according to the Euclidean distance of the key vectors from $f(c)$.
The set of nearest neighbors induces a distribution over the tokens $w_i$ appearing as values based on a softmax over the negative distance of their keys $f(c_i)$ from $f(c)$:
$$P_{k\text{NN}} (v \mid c)  \propto   \sum_{(f(c_i), w_i)} \mathds{1}_{v = w_i} e^{\frac{- || f(c_i) - f(c) ||}{T}}$$
where $T$ is a temperature parameter to control peakiness of the resulting distribution. 

% \todo{we expand }
We can then interpolate this with the original language model as follows:
\begin{equation} \label{eq:knnlm}
P_{k\text{NN-LM}}(v \mid c) =
  (1-\lambda) P_\text{LM}(v | c)
  + \lambda P_{k\text{NN}} (v | c).
\end{equation}
The hyperparameters for the $k$NN-LM approach are the number $k$ of nearest neighbors, the interpolation constant $\lambda$, the temperature $T$, and the choice of datastore.

In this work, for tasks with static output label sets (e.g., sentiment as opposed to multiple-choice QA), we filter the datastore for each task to only include tokens that appear in the output vocabulary of our verbalizer.
Using the $k$NN-LM to determine a probability distribution over continuations of the input $\mathbf{x}$, we can assign probabilities to the task's output labels using our verbalizers as in \autoref{eq:prompt-label-prob}.

%Formally, given a example pair $(c_i, w_i)$ from a text corpus $D$ where $c_i$ is a leftward context and $w_i$ is its next token, a pretrained language model can map $c_i$ to its hidden representation space by running a single forward pass. We denote $f(c_i)$ as the language model's representation of the leftward context $c$. A datastore is constructed by taking $f(c)$ as the key and its next token $w$ as the value. Different from kNN-LM \citep{Khandelwal2020Generalization} that save every token from the text corpora in datastore, we construct a task-specific datastore.
%For each task with label words $\cup_{y \in Y} V_y$,
%we only include example pairs where $w_i$ belongs to the set of label words ($w_i \in \cup_{y \in Y} V_y$) in the datastore.
%Thus, the final task-specific datastore $(K, V)$ is defined as:
%$$(K, V) = \{(f(c_i), w_i ) | (c_i, w_i) \in D \land w_i \in \cup_{y \in Y} V_y   \}$$
%
%\noindent \textbf{Querying datastore}
%To get model prediction on the test example $x$, we run a language model forward pass on $x_{input}$ to generate its next token probability distribution $P_L(v | x_{input})$ as well as the hidden representation $f(x_{input})$. Then $f(x_{input})$ is utilized to query the datastore for k-nearest neighbors $N_x = \{(f(c_i), w_i), i \in \{1, 2...k \}\}$ based on euclidean distance $d$. The k-nearest neighbor distribution over a label word $v \in \cup_{y \in Y} V_y$ is defined based on a softmax of their negative distance:
%$$P_{kNN} (v | x)  \propto   \sum_{(f(c_i), w_i)} \mathds{1}_{v = f(c_i)} e^{\frac{-d(f(c_i), f(x_{input}))}{T}}$$
%where $T$ is a temperature parameter to control peakness of the resulting distribution. 
%
%\noindent \textbf{Interpolation}
%The final distribution over a label word $v$ given a text example $x$ is defined as a weighted combination of language model's probability distributions and kNN distributions using a tuned parameter $\lambda$:
%$$ P(v|x_{input}) =  {(1-\lambda)P_L(v | x_{input}) + \lambda P_{kNN} (v | x_{input})}$$





% \noindent \textbf{Querying datastore}


\subsection{Zero-shot calibration}
\label{sec:scoring}
% \todo{[Julian: I don't think we need this paragraph here. Instead we should just briefly recap how domain-conditional PMI works and explain how we use it as a decision rule. Actually I can't remember: do you apply it over the vocabulary items prior to running them through the verbalizer? Or do you apply it to the output labels after running the LM outputs through the verbalizer? I'm having a hard time following the second half of this subsection.]}
% \noindent \textbf{kNN-enhanced word prior}

Motivated by the fact that language models suffer from surface from competition between different strings, \citeauthor{holtzman-etal-2021-surface} proposes using Pointwise Mutual Information(PMI) to calibrate the predicted distribution $P_{LM}(v|c)$ using a prior distribution $P_{LM}(v|c_{domain})$:
% $$\tilde{P}_{LM}(v \mid c) = \frac{P_{LM}(v \mid c)}{P_{LM}(v \mid c_{domain})}$$
$$ PMI(v, c) = \frac{P_{LM}(v \mid c)}{P_{LM}(v \mid c_{domain})}$$
where $c_{domain}$ is a short domain-relevant string, usually just the ending of the prompt. (e.g: $c_{domain}$ = "It was" for the example shown in Figure~\ref{fig:knn_prompt}). We also observe the surface form competition problem when retrieving target words from the datastore; some label words are more likely to be retrieved than the others, resulting in a biased prediction. To mitigate the drastic difference in prior probabilities of label words, we propose a kNN-enhanced prior $P_{\text{kNN-LM}}(v \mid c_{domain})$ using \autoref{eq:knnlm}.
to calibrate the interpolated distribution. By combining prompting, kNN-LM and zero-shot calibration, we define the final scoring function \ourmodel~for a given input $\mathbf{x}$:
\begin{equation*}
P_{\ourmodel}(y \mid x) \propto 
\sum_{\mathbf{z} \in \mathbf{Z}_y} \frac{P_\text{kNN-LM}(\mathbf{z} \mid p(\mathbf{x}))}{P_{\text{kNN-LM}}(\mathbf{z} \mid \mathbf{x}_{domain})}
\end{equation*}


% \begin{equation} \label{eq:prompt-label-prob}
% P(y \mid \mathbf{x}) = \frac{\sum_{\mathbf{z} \in \mathbf{Z}_y} P_\text{LM}(\mathbf{z} \mid p(\mathbf{x}))}{\sum_{y \in Y} \sum_{\mathbf{z} \in \mathbf{Z}_y} P_\text{LM}(\mathbf{z} \mid p(\mathbf{x}))}.
% \end{equation}

% Given a prompt , the prected label $y$ is 


% $P_{LM}(v)$ is the prior probability of the label word approximating by $P_{LM}(v|c_{domain})$. 



% Previous works~\cite{holtzman-etal-2021-surface, zhao2021calibrate} have shown that language models suffer from common token bias, which leads the models to prefer label words that are more frequent in its pretraining data. We also observe a similar phenomenon when retrieving target words from the datastore; some label words are more likely to be retrieved than the others, resulting in a biased prediction. 
% To mitigate the drastic difference in the prior probabilities of label words, we define a new kNN-enhanced word prior~\cite{holtzman-etal-2021-surface} to calibrate the predicted distribution. As suggested by \citeauthor{holtzman-etal-2021-surface}, language models are not trained to produce unconditional estimates of label words. We follow the same procedure and incorporate domain information into computing the prior. Therefore, the kNN-enhanced word prior of a label word $v$ is defined as:
% $$P(v|x_{domain}) =  (1-\lambda)P_L(v | x_{domain}) + \lambda P_{kNN} (v | x_{domain})$$
% where $x_{domain}$ is a short domain-relevant string. For example, ....

% $$
% P^{PMI}_{L} (v | x_{input}) = \frac{P_{L} (v | x_{input})}{P_{L}(v|x_{domain})}
% $$

% \subsection{Word Probability to Label Decision}
% The final problem is to design a score function that can not only map label word probabilities to the decision of labels but also take kNN-enhanced word prior into consideration. 
% Therefore, given a label $y$ and its associated label word set $V_y$, we leverage Equation~\ref{eq:sum} to define a label probability $P(y|x_{input}) =  \sum_{v \in V_y} P(v | x_{input}) $ and a domain conditional label prior probability $P(y|x_{domain}) =  \sum_{v \in V_y} P(v | x_{domain})$. 
% Following Pointwise Mutual Information, we factor out the label prior probability from the label probability to form the final score $S(y|x)$.
% \begin{align*}
% & S(y|x) = \frac{P(y|x_{input})}{P(y|x_{domain})} \\
% & = \frac{ \sum_{v \in V_y} P(v | x_{input}) }{  \sum_{v \in V_y} P(v | x_{domain})  } \\
% &= \frac{\sum_{v \in V_y}{(1-\lambda)P_L(v | x_{input}) + \lambda P_{kNN} (v | x_{input})}}{\sum_{v \in V_y}{(1-\lambda) P_{L}(v|x_{domain})} + \lambda {P_{kNN}(v|x_{domain})})}
% \end{align*}

% \subsection{Special case of multiple tokens in a label word}



% in consideration of contextualized prior. Moreover, we need to take into 
% To measure the conditional prior over a label, we define a 

% \begin{align*}
%     P(y|x_{domain}) = \sum_{v \in V_y} P(v | x_{domain}) = (1-\lambda)P_L(v | x_{domain}) + \lambda P_{kNN} (v | x_{domain})
% \end{align*}

% Therefore, we first define a contextualized prior over 
% \noindent \textbf{kNN-enhanced contextualized prior}






% \subsection{Inference}


% \subsection{score function without calibration}
% % We denote the final probability over a label word $v$ given $x_{input}$ as $P(v | x_{input})$ such that
% % $$P(v | x_{input}) = (1-\lambda)P_L(v | x_{input}) + \lambda P_{kNN} (v | x)$$
% $$score(y|x_{input}) =P(y|x_{input}) =  \sum_{v \in V_y}{(1-\lambda)P_L(v | x_{input}) + \lambda P_{kNN} (v | x)}$$

% % \subsection{score function with calibration 1}
% % $$score(y|x_{input}) =\sum_{v \in V_y}{\frac{(1-\lambda)P_L(v | x_{input}) + \lambda P_{kNN} (v | x)}{P_{L}(v|x_{domain})}}$$
% % problem: not a valid probability distribution inside sum

% \subsection{score function with calibration}
% We define a domain conditional prior probability over a set of label words $P(y|x_{domain}) = \sum_{v \in V_y}{P_{L}(v|x_{domain})}  $ 

% $$score(y|x_{input}) = \frac{P(y|x_{input})}{P(y|x_{domain})} = \frac{\sum_{v \in V_y}{(1-\lambda)P_L(v | x_{input}) + \lambda P_{kNN} (v | x)}}{\sum_{v \in V_y}{P_{L}(v|x_{domain})})}$$ 

% % \subsection{score function with calibration 3}
% why we use $P_L(v | x_{input})$ to calibrate $P_{kNN} (v | x)$ 



% \newpage
% ~\newpage




% A model with fewer parameters can 
% A smaller model take small model 

% Most of the benefit can be realized with a retrieval model with fewer parameters. 


% with label words.  

% none of previous works study if the performance of retrieval augmented language models can translate to downstream tasks. 
% \todo{Not sure if I explain the score function clearly}

% \todo{kNN-LM vs. \ourmodel}


==> sections/notes.tex <==
\section{A probability distribution over datastore}
It is hard to give a well-defined probabilistic meaning to k-NN method, so we approach the problem in the following way. We assume the datastore implicitly defines a probability distribution $\Pr_{DS}$ over embedding and next token pairs $\{(E, T)\}$. Given a context $c$ and its embedding $e_c$, the goal is to compute the following query:
\begin{equation}
\label{eq:query}
{\Pr}_{DS} (T = good | E = e_c)
\end{equation}
We apply Bayes Rule:

\begin{align*}
& \frac{{\Pr}_{DS} (E = e_c | T = good) {\Pr}_{DS} (T = good)}{{\Pr_{DS}(E = e_c)}} \\
& \propto {\Pr}_{DS} (E = e_c | T = good) {\Pr}_{DS} (T = good)
\end{align*}

Now we want to model ${\Pr}_{DS} (E = e_c | T = good)$ and ${\Pr}_{DS} (T = good)$. For ${\Pr}_{DS} (T = good)$, we can count the frequency of $T = good$ in datastore. 

For ${\Pr}_{DS} (E = e_c | T = good)$, we can collect pairs $\{(e_i, good)\}$ from datastore and ``learn'' the distribution ${\Pr}_{DS} (E | T = good)$ given the context embeddings $\{e_i\}$. Then we can compute query~\ref{eq:query}. Now the problem reduces to learning a probabilistic model given $\{e_i\}$. The model can be as simple as a (mixture over) multivariate Gaussian distribution or it can be a more complicated model like normalizing flows.

Similarly we can compute ${\Pr}_{DS} (T = bad | E = e_c)$, and we can make prediction by comparing it against ${\Pr}_{DS} (T = good | E = e_c)$. Note that ${\Pr}_{DS} (E | T = bad)$ and ${\Pr}_{DS} (E | T = good)$ should be separate models.

For an alternative view of this problem, suppose datastore stores the context and next token pairs $\{(C, T)\}$ instead of $\{(E, T\}$, we can even use a language model to model ${\Pr}_{DS} (C = c | T = good)$.

==> tables/main_table_tmp.tex <==
% \begin{table*}[htbp]
% \small
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
% & \multicolumn{2}{c}{Params} & \multicolumn{2}{c}{125M} & \multicolumn{2}{c}{350M} & \multicolumn{2}{c}{760M} & \multicolumn{2}{c}{1.6B} \\
% & \multicolumn{2}{c}{Datasets} & LM & kNN & LM & knn & LM & knn  & LM & knn \\
% \hline
% Datastore domain & \multicolumn{10}{c}{Classifcation} \\
% \hline
% \multirow{2}{*}{ wiki } & Topic classifcation & AGNews & 63 & 65.3 & 64.4 & 66.3 & 64.1 & 66.2 & 65.4 & 66.4 \\
% & & DBPedia & 74.1 & 83.2 & 75.5 & 83 & 75.7 & 83.1 & 76.6 & 83.5 \\
% & & & & & & & & & & \\
% wiki & NLI & RTE & 49.8 & 45.2 & 54.9 & 51.4 & 54.2 & 52.2 & 48.5 & 40.3 \\
% & & & & & & & & & & \\
% \multirow{3}{*}{ review corpus } & Sentiment analysis & SST-2 & 67.1 & 72.5 & 86.2 & 86.8 & 85.6 & 86.4 & 87.4 & 87.9 \\
% & & MR & 61.6 & 67 & 66.4 & 69.4 & 67.1 & 68.3 & 69.2 & 70.3 \\
% & & Hyperpartisan & 63.8 & 67.4 & 70 & 69.1 & 69.4 & 70.3 & 71.6 & 73.2 \\
% & & & & & & & & & & \\
% \hline
% & \multicolumn{10}{c}{Generation } \\
% \hline
% \multirow{5}{*}{ wiki } & QA & OBQA & 32.4 & 37.1 & 38.6 & 41.3 & 43.2 & 45.6 & 46 & 47.2 \\
% & & CQA & 36.4 & 40.2 & 41.8 & 44.3 & 44.5 & 45.2 & 47.8 & 49.4 \\
% & & BoolQ & 59.7 & 47.3 & 49.7 & 45.6 & 46.1 & 43.1 & 49.5 & 40.2 \\
% & Information Retrieval & LAMA & - & - & - & - & 14 & 22.1 & 23.5 & 34.3 \\
% & & MIT-D & - & - & - & - & 12.7 & 20.8 & 18.7 & 25.5 \\
% \end{tabular}
% \end{table*}

\begin{table*}[htbp]
\scriptsize
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{3}{*}{ Params } & \multicolumn{8}{c|}{125M } & \multicolumn{8}{c}{350M} \\
& \multicolumn{2}{c|}{Base}  & \multicolumn{2}{c|}{Pretrain} & \multicolumn{2}{c|}{Demo} & \multicolumn{2}{c|}{\ourmodel} & \multicolumn{2}{c|}{Base} & \multicolumn{2}{c|}{Pretrain} & \multicolumn{2}{c|}{Demo} & \multicolumn{2}{c}{\ourmodel} \\
& LM & PMI & LM & PMI & LM & PMI & LM & $PMI_{kNN}$ & LM & PMI & LM & PMI & LM & PMI & LM & $PMI_{kNN}$ \\
\hline
RTE & 51.2 & 49.1 & & & & & 54.8 & 53.7 & 53.1 & 54.5 & & & & & 55.2 & 55.2 \\
CQA & 25.5 & 36.4 & & & & & 31.1 & 39.3 & 30.9 & 41.8 & & & & & 33.2 & 44.2 \\
OBQA & 16.4 & 32.4 & & & & & 18.4 & 35.4 & 18.6 & 38.6 & & & & & 21.3 & 40.0 \\
LAMA & 11.3 & 19.5 & 15.2 & 23.8 & & & 16.4 & 24.1 & 13.2 & 21.9 & 17.3 & 24.5 & & & 17.1 & 24.3 \\
SST-2 & 63.9 & 78.4 & 55.2 & 80.1 & 65.4 & 78.5 & 75.5 & 79.6 & 68.4 & 76.7 & 59.3 & 80.3 & 68.2 & 79.2 & 80.5 & 80.6 \\
IMDB & 80.8 & 81.4 & 63.5 & 84.7 & 73.3 & 75.4 & 82.2 & 83.5 & 85.5 & 86.1 & 79.2 & 89.3 & 75.1 & 78.6 & 87.7 & 88.8 \\
CR & 54.5 & 71.8 & 50.9 & 82.8 & 48.6 & 71.2 & 62.9 & 82.0 & 56.6 & 69.2 & 52.1 & 85.5 & 52.4 & 60.1 & 71.6 & 84.3 \\
MR & 53.5 & 67.9 & 50.4 & 62.1 & 57.1 & 68.4 & 64.8 & 72.1 & 60.8 & 73.5 & 53.1 & 66.7 & 57.3 & 67.2 & 66.1 & 77.9 \\
HYP & 58.4 & 58.4 & 60.2 & 66.7 & & & 66.1 & 64.6 & 58.4 & 61.5 & 62.2 & 67.4 & & & 66.1 & 64.6 \\
AGN & 58.6 & 64.9 & 59.5 & 66.4 & & & 62.3 & 67.5 & 71.4 & 71.4 & 72.3 & 72.6 & & & 72.6 & 74.4 \\
\hline
Avg. & 47.4 & 56.0 & 50.7 & 66.7 & & & 53.5 & 60.2 & 51.7 & 59.5 & 56.5 & 69.5 & 63.3 & 71.3 & 57.1 & 63.4 \\
\end{tabular}

% imdb adapt to unlabeled data, use task-datastore from don't stop pretraining, change the datastore, rte from NLI: more relevant corpus --> better improvement 
% task relevant data from domain data: check the retrieved texts, what makes a good retrieved contexts 
% plot: datastore size/domain changes - performance 
% try sewon's method: example + prompt + label word 

\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc}
\midrule
\multirow{3}{*}{ Params } & \multicolumn{8}{c|}{760M} & \multicolumn{8}{c}{1.6B} \\  
& \multicolumn{2}{c|}{Base}  & \multicolumn{2}{c|}{Pretrain} & \multicolumn{2}{c|}{Demo} & \multicolumn{2}{c|}{\ourmodel} & \multicolumn{2}{c|}{Base} & \multicolumn{2}{c|}{Pretrain} & \multicolumn{2}{c|}{Demo} & \multicolumn{2}{c}{\ourmodel} \\
& LM & PMI & LM & PMI & LM & PMI & LM & $PMI_{kNN}$ & LM & PMI & LM & PMI & LM & PMI & LM & $PMI_{kNN}$ \\
\hline
RTE & 52.7 & 54.5 & & & & & 56.7 & 57.0 & 47.6 & 53.4 & & & & & 55.2 & 55.2 \\
CQA & 33.3 & 44.5 & & & & & 37.2 & 48.3 & 38.6 & 47.8 & & & & & 42.2 & 49.4 \\
OBQA & 19.4 & 43.2 & & & & & 21.2 & 46.6 & 22.4 & 46.0 & & & & & 24.0 & 48.1 \\
LAMA & 12.6 & 20.1 & 17.5 & 25.0 & & & 18.3 & 26.1 & 14.0 & 22.7 & & & & & 18.0 & 25.9 \\
SST-2 & 58.5 & 81.4 & 55.7 & 70.6 & 62.2 & 71.4 & 77.7 & 81.6 & 59.9 & 85.3 & 57.8 & 78.0 & 66.9 & 75.6 & 74.1 & 85.6 \\
IMDB & 85.5 & 83.0 & 72.6 & 80.8 & 76.9 & 78.4 & 87.1 & 88.0 & 86.7 & 88.0 & 79.0 & 91.8 & 79.4 & 78.2 & 88.4 & 90.7 \\
CR & 54.3 & 64.4 & 52.3 & 85.2 & 51.5 & 62.3 & 71.4 & 84.0 & 55.0 & 66.7 & 53.3 & 83.5 & 53.3 & 62.5 & 72.1 & 84.4 \\
MR & 58.8 & 70.8 & 56.0 & 69.4 & 60.2 & 71.4 & 69.9 & 77.2 & 62.7 & 75.3 & 50.3 & 72.3 & 61.5 & 73.1 & 70.8 & 80.0 \\
HYP & 58.3 & 58.4 & 61.4 & 67.0 & & & 64.2 & 66.1 & 58.4 & 63.0 & 64.5 & 68.2 & & & 66.1 & 67.6 \\
AGN & 68.1 & 76.7 & 72.2 & 75.4 & & & 74.0 & 77.1 & 73.6 & 73.2 & 74.3 & 76.2 & & & 76.1 & 75.4 \\
\hline
Avg. & 50.2 & 59.7 & 55.4 & 67.6 & 62.7 & 70.9 & 57.8 & 65.2 & 51.9 & 62.1 & 63.2 & 78.3 & 65.3 & 72.4 & 58.7 & 66.2 \\
\bottomrule
\end{tabular}
\caption{\ourmodel~improves accuracy of GPT2 (Base) across a range of tasks. We use accuracy as a metric for all datasets.}  \label{main_table}

\end{table*}

==> tables/tapt.tex <==

\begin{table}[t]
\centering
\small
\begin{tabular}{cccc}
\toprule
Task & Data & Size & Accuracy \\
\hline
\multirow{2}{*}{ MR } & General & 465M & 81.5 \\
& Task & 0.2M & 81.2 \\
\hline
\multirow{2}{*}{ AGN } & General & 465M & 77.3 \\
& Task & 6M & 79.1 \\
\hline
\multirow{2}{*}{ RT } & General & 465M & 83.8 \\
& Task & 0.2M & 81.6 \\
\bottomrule
\end{tabular}
\caption{Domain adaptation using \ourmodel. Instead of a general-purpose corpus, \ourmodel~uses a domain-specific datastore to adapt the model. DAPT relies on calibrated distribution to make predictions.
}  \label{tapt_table}
\end{table}
